Efficient Off-Grid Bayesian Parameter Estimation for Kronecker-Structured Signals

This work studies the problem of jointly estimating unknown parameters from Kronecker-structured multidimensional signals, which arises in applications like intelligent reflecting surface (IRS)-aided channel estimation. Exploiting the Kronecker structure, we decompose the estimation problem into smaller, independent subproblems across each dimension. Each subproblem is posed as a sparse recovery problem using basis expansion and solved using a novel off-grid sparse Bayesian learning (SBL)-based algorithm. Additionally, we derive probabilistic error bounds for the decomposition, quantify its denoising effect, and provide convergence analysis for off-grid SBL. Our simulations show that applying the algorithm to IRS-aided channel estimation improves accuracy and runtime compared to state-of-the-art methods through the low-complexity and denoising benefits of the decomposition step and the high-resolution estimation capabilities of off-grid SBL.

==> utils/basestation.tex <==

% chktex-file 1
% chktex-file 27

\makeatletter


% The keys that the user can provide are all the keys below.

% Keys for the Beam shape
\pgfkeys{
  /pgf/.cd,
  % The 4 following options control the proportion of shapewidth/shapeheight for
  % the control points of the beam -> The must be greater than zero
  control point 1 x/.initial=0.35,
  control point 1 y/.initial=1.0,
  control point 2 x/.initial=0.5,
  control point 2 y/.initial=0.25,
}

% Keys for the UserTerminal shape
\pgfkeys{
  /pgf/.cd,
  button fill color/.initial=white,
  screen fill color/.initial=white,
}


% Represents a "beam", which is constructed using two Bézier curves.
% The two control points can be controlled by passing the
% "control point 1 x/control point 1 y/control point 2 x/control point 2 y"
% parameters.
\pgfdeclareshape{Beam}{

  % xxxxxxxxxx Define some saved macros xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }

  \savedmacro\firstpointxprop{
    \def\firstpointxprop{\pgfkeysvalueof{/pgf/control point 1 x}}
  }
  \savedmacro\firstpointyprop{
    \def\firstpointyprop{\pgfkeysvalueof{/pgf/control point 1 y}}
  }
  \savedmacro\secondpointxprop{
    \def\secondpointxprop{\pgfkeysvalueof{/pgf/control point 2 x}}
  }
  \savedmacro\secondpointyprop{
    \def\secondpointyprop{\pgfkeysvalueof{/pgf/control point 2 y}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  \savedanchor\startpoint{%
    \pgfmathsetlength\pgf@x{-0.5*\shapewidth}
    \pgfmathsetlength\pgf@y{0}
  }

  \savedanchor\endpoint{%
    \pgfmathsetlength\pgf@x{0.5*\shapewidth}
    \pgfmathsetlength\pgf@y{0}
  }

  % \savedanchor\centerpoint{%
  %   \pgf@x=0%
  %   \pgf@y=0%
  % }

  % Control point anchors
  \savedanchor\firstcontrolpointtop{%
    \pgfmathsetlength\pgf@x{\firstpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{\firstpointyprop*\shapeheight}
  }

  \savedanchor\secondcontrolpointtop{%
    \pgfmathsetlength\pgf@x{\secondpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{\secondpointyprop*\shapeheight}
  }

  \savedanchor\firstcontrolpointbottom{%
    \pgfmathsetlength\pgf@x{\firstpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{-\firstpointyprop*\shapeheight}
  }

  \savedanchor\secondcontrolpointbottom{%
    \pgfmathsetlength\pgf@x{\secondpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{-\secondpointyprop*\shapeheight}
  }

  % xxxxxxxxxx Define regular anchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{center}{\startpoint}
  \anchor{start}{\startpoint}
  \anchor{end}{\endpoint}
  \anchor{main region}{
    \endpoint
    \pgfmathsetlength\pgf@x{\pgf@x-0.25*\shapewidth}
  }
  \anchor{top control point 1}{\firstcontrolpointtop}
  \anchor{top control point 2}{\secondcontrolpointtop}
  \anchor{bottom control point 1}{\firstcontrolpointbottom}
  \anchor{bottom control point 2}{\secondcontrolpointbottom}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  \inheritanchorborder[from=rectangle]

  % xxxxxxxxxx Draw the background path xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    \begin{pgfscope}
      \pgfmoveto{\startpoint}
      \pgfcurveto{\firstcontrolpointtop}{\secondcontrolpointtop}{\endpoint}
      \pgfcurveto{\secondcontrolpointbottom}{\firstcontrolpointbottom}{\startpoint}
      \pgfpathclose
      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx UserTerminal Shape xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{UserTerminal}{

  % xxxxxxxxxx First we define some savedmacros xxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Macros and savedanchors common to UserTerminal and BaseStation Shapes
  \savedanchor{\center}{
    \pgf@x=0pt
    \pgf@y=0pt
  }

  % Note that pgf provides the text macros \pgfshapeminwidth and
  % pgfshapeminheight that store the minim width and minimum height,
  % respectivelly. Note that They are "TEXT macros" and not
  % "lengths". Calling them simple
  % replaces for the text.
  \savedanchor{\northeast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.5\pgf@ya
    % NOTE: We can't use 0.5\pgfshapeminwidth directly because the minimum
    % width is stored in a "plain text macro". If minimum width is 2cm, for
    % instance, and we write "\pgf@x=.5\pgfshapeminwidth" then \pgf@x would
    % be set to 0.52cm, which is not what we want. See the explanation for
    % \savedanchor in the pgfmanual (page 627).
  }

  \savedanchor{\southwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=-0.5\pgf@ya
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Savedanchors specific to the UserTerminal shape
  \savedanchor{\screennortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.45\pgf@xa
    \pgf@y=0.45\pgf@ya
  }

  \savedanchor{\screensouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.45\pgf@xa
    \pgf@y=-0.35\pgf@ya
  }

  \savedanchor{\buttonsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=-0.425\pgf@ya
    \advance\pgf@x by -0.15\pgf@xa
    \advance\pgf@y by -0.04\pgf@ya
  }

  \savedanchor{\buttonnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=-0.425\pgf@ya
    \advance\pgf@x by 0.15\pgf@xa
    \advance\pgf@y by 0.04\pgf@ya
  }

  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from rectangle xxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from rectangle xxxxxxxxxxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % rectangle shape (even thought the northeast and southwest saved anchors
  % in the rectangle shape are different from ours).
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{text}
  {
    % This will get the center of the screen
    \pgfpointlineattime{0.5}{\screensouthwest}{\screennortheast}
    % Lets put the center of the text in the center of the screen
    \advance\pgf@x by -0.5\wd\pgfnodeparttextbox
    \advance\pgf@y by -0.5\ht\pgfnodeparttextbox
  }

  \anchor{button}{
    \pgfpointlineattime{0.5}{\buttonsouthwest}{\buttonnortheast}
  }

  \anchor{screen}{
    \pgfpointlineattime{0.5}{\screensouthwest}{\screennortheast}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Scope for Terminal Body
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      % '\pgfshapeminheight' cannot be used directly; or if you want to use it directly use the '*' for multiplication
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfpathrectanglecorners
      {\southwest}
      {\northeast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the terminal Screen
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/screen fill color}}
      %\pgfsetfillcolor{white}
      \pgfpathrectanglecorners
      {\screensouthwest}
      {\screennortheast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the button
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.009\pgf@ya}{0.009\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/button fill color}}
      %\pgfsetfillcolor{white}
      \pgfpathrectanglecorners
      {\buttonsouthwest}
      {\buttonnortheast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx BaseStationSimple xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{BaseStationSimple}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from UserTerminal. We only need northeast and
  % southwest, but we can't choose which ones to inherit.
  \inheritsavedanchors[from=UserTerminal]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  \savedanchor{\BaseAsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.5\pgf@ya
    \pgf@x=-0.12\pgf@xa
  }

  \savedanchor{\BaseAnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.30\pgf@ya
    \pgf@x=0.12\pgf@xa
  }

  % Maybe I don't need this savedanchor
  \savedanchor{\MiddleAntennasouth}{
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\AntennaConnectorsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=0.38\pgf@ya
  }

  \savedanchor{\AntennaConnectornortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.42\pgf@ya
  }

  \savedanchor{\MiddleAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.15\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\MiddleAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.15\pgf@xa
    \pgf@y=0.5\pgf@ya
  }

  \savedanchor{\LeftAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\LeftAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.25\pgf@xa
    \pgf@y=0.5\pgf@ya
  }

  \savedanchor{\RightAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.25\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\RightAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.5\pgf@ya
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from UserTerminal xxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=UserTerminal]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from UserTerminal xxxxxxxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % UserTerminal shape (even thought the northeast and southwest saved anchors
  % in the UserTerminal shape are different from ours).
  \inheritanchor[from=UserTerminal]{center}
  \inheritanchor[from=UserTerminal]{north}
  \inheritanchor[from=UserTerminal]{east}
  \inheritanchor[from=UserTerminal]{south}
  \inheritanchor[from=UserTerminal]{west}
  \inheritanchor[from=UserTerminal]{north east}
  \inheritanchor[from=UserTerminal]{north west}
  \inheritanchor[from=UserTerminal]{south west}
  \inheritanchor[from=UserTerminal]{south east}
  \inheritanchor[from=rectangle]{text}
  \anchor{antenna right}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
  }
  \anchor{antenna left}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
    \pgfmathsetlength\pgf@x{-\pgf@x}
  }
  \anchor{antenna center}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
    \pgfmathsetlength\pgf@x{0}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the "behind background" xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % The base of the antenna will be in the behindbackgroundpath while the
  % antennas will be in the backgroundpath.
  \behindbackgroundpath{
    % Scope for the Base
    \begin{pgfscope}
      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseAsouthwest}
      {\BaseAnortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % The base of the antenna will be in the behindbackgroundpath while the
  % antennas will be in the backgroundpath. The main reason for this
  % separation is that this code here will be inherited in the
  % "BaseStation" shape that we will define later.
  \backgroundpath{
    % Scope for the antenna connector
    \begin{pgfscope}
      % Draw Antenna connector
      \pgfpathrectanglecorners
      {\AntennaConnectorsouthwest}
      {\AntennaConnectornortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the antennas
    \begin{pgfscope}
      % Draw the middle antenna
      \pgfpathrectanglecorners
      {\MiddleAntennasouthwest}
      {\MiddleAntennanortheast}

      % Draw the Left antenna
      \pgfpathrectanglecorners
      {\LeftAntennasouthwest}
      {\LeftAntennanortheast}

      % Draw the Right antenna
      \pgfpathrectanglecorners
      {\RightAntennasouthwest}
      {\RightAntennanortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx BaseStation Shape xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{BaseStation}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from BaseStationSimple.
  \inheritsavedanchors[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  \savedanchor{\BaseAsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.5\pgf@ya
    \pgf@x=-0.2\pgf@xa
  }

  \savedanchor{\BaseAnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.05\pgf@ya
    \pgf@x=0.2\pgf@xa
  }

  \savedanchor{\BaseBsoutheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.05\pgf@ya
    \pgf@x=0.15\pgf@xa
  }

  \savedanchor{\BaseBnorthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.15\pgf@ya
    \pgf@x=-0.15\pgf@xa
  }

  \savedanchor{\BaseCsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.15\pgf@ya
    \pgf@x=-0.1\pgf@xa
  }

  \savedanchor{\BaseCnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.30\pgf@ya
    \pgf@x=0.1\pgf@xa
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from BaseStationSimple xxxxxxxxxxxxxxx
  \inheritanchorborder[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from BaseStationSimple xxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % BaseStationSimple shape (even thought the northeast and southwest saved anchors
  % in the BaseStationSimple shape are different from ours)..
  \inheritanchor[from=BaseStationSimple]{center}
  \inheritanchor[from=BaseStationSimple]{north}
  \inheritanchor[from=BaseStationSimple]{east}
  \inheritanchor[from=BaseStationSimple]{south}
  \inheritanchor[from=BaseStationSimple]{west}
  \inheritanchor[from=BaseStationSimple]{north east}
  \inheritanchor[from=BaseStationSimple]{north west}
  \inheritanchor[from=BaseStationSimple]{south west}
  \inheritanchor[from=BaseStationSimple]{south east}
  \inheritanchor[from=BaseStationSimple]{antenna right}
  \inheritanchor[from=BaseStationSimple]{antenna left}
  \inheritanchor[from=BaseStationSimple]{antenna center}
  \inheritanchor[from=rectangle]{text}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the "behind background" xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \behindbackgroundpath{
    % Scope for the Base
    \begin{pgfscope}
      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseAsouthwest}
      {\BaseAnortheast}

      % Draw the middle base
      \pgfpathrectanglecorners
      {\BaseBsoutheast}
      {\BaseBnorthwest}

      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseCsouthwest}
      {\BaseCnortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxx Inherit the background path from BaseStationSimple xxxxxxxxxxx
  \inheritbackgroundpath[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "testbasestation.tex"
%%% TeX-PDF-mode: t
%%% End:

==> utils/irs.tex <==
% chktex-file 1
% chktex-file 27

\makeatletter

% The keys that the user can provide are all the keys below.

\pgfkeys{
  /pgf/.cd,
  element fill color/.initial=white,
}


\pgfdeclareshape{IRS}{

  % xxxxxxxxxx Define some saved macros xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Saved Anchors for each element top left and bottom right xxxxxxxx
  % 
  % The IRS elements are named with single capital letters in a
  % rowwise fashion. That is, element 1-1 is A, element 1-2 is B, and
  % so on.
  % 
  % The width/height of each IRS element is 0.2 of the full IRS
  % width/height. The spacing between elements is 0.04 of the width/height.
  
  % First row
  \savedanchor\elementAtopleft{%
    \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementAbottomright{%
    \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }
  
  \savedanchor\elementBtopleft{%
    \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementBbottomright{%
    \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

  \savedanchor\elementCtopleft{%
    \pgfmathsetlength\pgf@x{0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementCbottomright{%
    \pgfmathsetlength\pgf@x{0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

  \savedanchor\elementDtopleft{%
    \pgfmathsetlength\pgf@x{0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementDbottomright{%
    \pgfmathsetlength\pgf@x{0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }
  
%   Cdots
  \savedanchor\elementctopleft{%
    \pgfmathsetlength\pgf@x{0.74*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementcbottomright{%
    \pgfmathsetlength\pgf@x{0.94*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

%   Second Row
  \savedanchor\elementEtopleft{%
    \pgfmathsetlength\pgf@x{0.74*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementEbottomright{%
    \pgfmathsetlength\pgf@x{0.94*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }
  
%   \savedanchor\elementFtopleft{%
%     \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.22*\shapeheight}
%   }

%   \savedanchor\elementFbottomright{%
%     \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.02*\shapeheight}
%   }

%   \savedanchor\elementGtopleft{%
%     \pgfmathsetlength\pgf@x{0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.22*\shapeheight}
%   }

%   \savedanchor\elementGbottomright{%
%     \pgfmathsetlength\pgf@x{0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.02*\shapeheight}
%   }

%   \savedanchor\elementHtopleft{%
%     \pgfmathsetlength\pgf@x{0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.22*\shapeheight}
%   }

%   \savedanchor\elementHbottomright{%
%     \pgfmathsetlength\pgf@x{0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.02*\shapeheight}
%   }

%   % Third Row
%   \savedanchor\elementItopleft{%
%     \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
%   }

%   \savedanchor\elementIbottomright{%
%     \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
%   }
  
%   \savedanchor\elementJtopleft{%
%     \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
%   }

%   \savedanchor\elementJbottomright{%
%     \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
%   }

%   \savedanchor\elementKtopleft{%
%     \pgfmathsetlength\pgf@x{0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
%   }

%   \savedanchor\elementKbottomright{%
%     \pgfmathsetlength\pgf@x{0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
%   }

%   \savedanchor\elementLtopleft{%
%     \pgfmathsetlength\pgf@x{0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
%   }

%   \savedanchor\elementLbottomright{%
%     \pgfmathsetlength\pgf@x{0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
%   }

%   % Forth Row
%   \savedanchor\elementMtopleft{%
%     \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
%   }

%   \savedanchor\elementMbottomright{%
%     \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
%   }
  
%   \savedanchor\elementNtopleft{%
%     \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
%   }

%   \savedanchor\elementNbottomright{%
%     \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
%   }

%   \savedanchor\elementOtopleft{%
%     \pgfmathsetlength\pgf@x{0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
%   }

%   \savedanchor\elementObottomright{%
%     \pgfmathsetlength\pgf@x{0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
%   }

%   \savedanchor\elementPtopleft{%
%     \pgfmathsetlength\pgf@x{0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
%   }

%   \savedanchor\elementPbottomright{%
%     \pgfmathsetlength\pgf@x{0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
%   }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  
  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from UserTerminal. We only need northeast and
  % southwest, but we can't choose which ones to inherit.
  \inheritsavedanchors[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  % NONE
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from UserTerminal xxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from UserTerminal xxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Draw the background path xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{

    % \begin{pgfscope}
    %   % \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    %   % '\pgfshapeminheight' cannot be used directly; or if you want to use it directly use the '*' for multiplication
    %   % \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
    %   \pgfpathrectanglecorners
    %   {\southwest}
    %   {\northeast}
    % %   \pgfusepath{stroke,fill}
    % \end{pgfscope}

    \begin{scope} % Scope for all IRS elements to make the rounded corners
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/element fill color}}
      
      % IRS Element 1-1
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementAtopleft}
        {\elementAbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-2
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementBtopleft}
        {\elementBbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-3
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementCtopleft}
        {\elementCbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-4
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementDtopleft}
        {\elementDbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 2-1
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementEtopleft}
        {\elementEbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}
      
      % Cdots
    %   \node[\elementctopleft] {$\tiny\cdots$}
      
    %   % IRS Element 2-2
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementFtopleft}
    %     {\elementFbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 2-3
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementGtopleft}
    %     {\elementGbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 2-4
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementHtopleft}
    %     {\elementHbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 3-1
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementItopleft}
    %     {\elementIbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 3-2
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementJtopleft}
    %     {\elementJbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 3-3
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementKtopleft}
    %     {\elementKbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 3-4
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementLtopleft}
    %     {\elementLbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 4-1
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementMtopleft}
    %     {\elementMbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 4-2
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementNtopleft}
    %     {\elementNbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 4-3
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementOtopleft}
    %     {\elementObottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 4-4
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementPtopleft}
    %     {\elementPbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}
    \end{scope}
    
    % \begin{pgfscope}
    %   \pgfmoveto{\startpoint}
    %   \pgfcurveto{\firstcontrolpointtop}{\secondcontrolpointtop}{\endpoint}
    %   \pgfcurveto{\secondcontrolpointbottom}{\firstcontrolpointbottom}{\startpoint}
    %   \pgfpathclose
    %   \pgfusepath{stroke,fill}
    % \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "test_irs.tex"
%%% End:

==> utils/mimoshapes.tex <==
% chktex-file 1
% chktex-file 27

% This file defines some new node shapes to use with tikz.
%
% The start code was taken and modified from the example in
% http://www.texample.net/tikz/examples/d-flip-flops-and-shift-register/
%
% The shapes defined here are:
% - mimoone
% - mimotwo
% - mimothree
% - mimoind
% - boxtwo
% - boxthree
%
% For the three first shapes you can epecify either the "right antennas" or
% "left antennas" option to indicate the antennas position. You can also
% change some distances by specifying the options "antenna offset",
% "antenna base height" and "antenna side" with some value.
%
% For the last two shapes you can change the appearance with the "circle
% fill color", "circle stroke color" and "circle radius" options.

\makeatletter

\newif\ifleftantennas

% The keys that the user can provide are all the keys below, except
% "leftantennas" (use the "right antennas" or "left antennas" keys instead)
\pgfkeys{
  /mimonode/leftantennas/.is if=leftantennas,
  /pgf/.cd,
  right antennas/.code={\pgfkeys{/mimonode/leftantennas=false}},
  left antennas/.code={\pgfkeys{/mimonode/leftantennas=true}},
  % minimum width/.initial=1.5cm,
  % minimum height/.initial=2cm,
  circle fill color/.initial=white,
  circle stroke color/.initial=black,
  circle radius/.initial=2mm,
  antenna offset/.initial=0.3cm,
  antenna yshift/.initial=0.cm,
  antenna base height/.initial=0.2 cm,
  antenna side/.initial=0.4cm,
}


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx Macro definitions xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

% Macro with the common code to draw an antenna. Before calling this macro
% (inside the backgroundpath or similar) you need to set the values of
% \pgf@x and \pgf@y to point to the start of the antenna.
\def\mimoshapesdrawantenna{
  % Store the current positions in \pgf@xa and \pgf@ya
  \pgf@xa=\pgf@x 
  \pgf@ya=\pgf@y
  \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}

  \advance\pgf@xa by \antennaoffset
  \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
  \pgfpathclose
  \pgfmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}

  % \pgf@xb and \pgf@yb will have the coordinate with the starting point to
  % draw the triangle
  \pgf@xb=\pgf@xa \pgf@yb=\pgf@ya
  \advance\pgf@yb by \antennabaseheight cm
  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  
  % See section "Internals of How Point Commands Work" of the pgf manual to
  % understand pgf@process
  \pgf@process{
    \pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\pgfpointpolar{60}{\pgfkeysvalueof{/pgf/antenna side}}}
  }
  \pgf@xc=\pgf@x 
  \pgf@yc=\pgf@y
  \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
  
  
  \pgf@process{
    \pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}{\pgfpointpolar{180}{\pgfkeysvalueof{/pgf/antenna side}}}
  }
  \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
  
  \pgf@process{
    \pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\pgfpointpolar{240}{\pgfkeysvalueof{/pgf/antenna side}}}
  }
  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
}


% Macro with the common code to draw the ellipses. Before calling this
% macro (inside the backgroundpath or similar) you need to set the values
% of \pgf@x and \pgf@y to point to the center of the ellipses.
\def\drawellipses{
  % Store the current positions in \pgf@xa and \pgf@ya
  \pgf@xa=\pgf@x 
  \advance\pgf@xa by \antennaoffset
  \pgf@ya=\pgf@y
  
  % See section "Internals of How Point Commands Work" of the pgf manual to
  % understand pgf@process
  \pgf@process{\pgfpathcircle{\pgfpoint{\pgf@xa}{\pgf@ya+\antennabaseheight-1pt}}{1pt}}
  \pgf@process{\pgfpathcircle{\pgfpoint{\pgf@xa}{\pgf@ya+\antennabaseheight+2pt}}{1pt}}
  \pgf@process{\pgfpathcircle{\pgfpoint{\pgf@xa}{\pgf@ya+\antennabaseheight+5pt}}{1pt}}
}


% The code to determine the x coordinate for the anchors in the start of
% each antenna is common for all antennas. Therefore, it is better to
% define a macro with it and just call the macro when define the respective
% savedanchor.
\def\antennaStartXCoordinate{
  % x position
  \ifleftantennas
  % Anchor position when the "left antennas" key is used
  \pgf@x=-.5\wd\pgfnodeparttextbox
  % Advance by the inner xsep
  \pgfmathsetlength\pgf@xc{-\pgfkeysvalueof{/pgf/inner xsep}}
  \advance\pgf@x by \pgf@xc%
  %
  % If the resulting x coordinate is lower the value required for the
  % minimum width then the value for the minimum width will be used instead
  \setlength{\pgf@xa}{-\pgfshapeminwidth}
  \ifdim\pgf@x>.5\pgf@xa
  \pgf@x=.5\pgf@xa
  \fi
  \else
  % Anchor position when the "left antennas" key is not used or when
  % the "right antennas" key is used.
  \pgf@x=.5\wd\pgfnodeparttextbox % width of the box
  \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}
  \advance\pgf@x by \pgf@xc%
  \setlength{\pgf@xa}{\pgfshapeminwidth}
  \ifdim\pgf@x<.5\pgf@xa
  \pgf@x=.5\pgf@xa
  \fi
  \fi
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx mimoone shape declaration xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{mimoone}{

  % xxxxxxxxxx First we define some savedmacros xxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\antennaoffset{
    \ifleftantennas
      \def\antennaoffset{-\pgfkeysvalueof{/pgf/antenna offset}}
    \else
      \def\antennaoffset{\pgfkeysvalueof{/pgf/antenna offset}}
    \fi
  }

  \savedmacro\antennabaseheight{
    \def\antennabaseheight{\pgfkeysvalueof{/pgf/antenna base height}}
  }

  \savedmacro\antennayshift{
    \def\antennayshift{\pgfkeysvalueof{/pgf/antenna yshift}}
  }

  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define the savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedanchor\northeast{%
    \pgf@y=.5\ht\pgfnodeparttextbox % height of the box, ignoring the depth
    \pgf@x=.5\wd\pgfnodeparttextbox % width of the box
    %
    % -----> Take the inner sep into account
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}
    \advance\pgf@x by \pgf@xc%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}
    \advance\pgf@y by \pgf@yc%
    % -----
    % Test if the minimum width and height are respected. If not, set it as
    % the minimum width/height.
    \setlength{\pgf@xa}{\shapewidth}
    \ifdim\pgf@x<.5\pgf@xa
    \pgf@x=.5\pgf@xa
    \fi
    \setlength{\pgf@ya}{\shapeheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    %
    % -----> Take the outer sep into account
    % Now that we have the values of x and y we could stop here. However,
    % in order to take into account the "outer sep" we need to add it to
    % the anchor position(the idea is that the anchor will be outside the
    % actual node (by the outer sep ammount). The default value of the
    % outer sep is half the length of a line. Note that we are including
    % the outer sep value in the anchor definition, but it should not be
    % taken into account when drawing the background. Therefore, we need to
    % remove this when drawing the rectangle box.
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }

  \savedanchor\southwest{%
    \pgf@y=-.5\ht\pgfnodeparttextbox % height of the box, ignoring the depth
    \pgf@x=-.5\wd\pgfnodeparttextbox % width of the box
    %
    % -----> Take the inner sep into account
    \pgfmathsetlength\pgf@xc{-\pgfkeysvalueof{/pgf/inner xsep}}
    \advance\pgf@x by \pgf@xc%
    \pgfmathsetlength\pgf@yc{-\pgfkeysvalueof{/pgf/inner ysep}}
    \advance\pgf@y by \pgf@yc%
    % 
    % Test if the minimum width and height are respected. If not, set it as
    % the minimum width/height.
    \setlength{\pgf@xa}{-\shapewidth}
    \ifdim\pgf@x>.5\pgf@xa
    \pgf@x=.5\pgf@xa
    \fi
    \setlength{\pgf@ya}{-\shapeheight}
    \ifdim\pgf@y>.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    %
    % -----> Take the outer sep into account (see comment in the northeast savedanchor)
    \pgfmathsetlength\pgf@xa{-\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength\pgf@ya{-\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }

  % This anchor position will depend if the "left antennas" option was
  % passed or not.
  \savedanchor{\anchorA}{
    % -----> y position for the first antenna
    \pgf@y=.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from rectangle xxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Inherit normal anchors from rectangle xxxxxxxxxxxxxxxxxxxxxx
  % We can inherit the "usual" from rectangle. They depend on the
  % "\southwest" and "\northeast" savedanchors but this will use our
  % version instead of the rectangle's version.
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{A}{
    \pgf@process{\anchorA}
  }

  \anchor{text}
  {
    \pgf@process{\pgfpointorigin}
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }
  
  % -----> Define some more useful anchors
  \anchor{first antenna base start}{
    \pgf@process{\anchorA}
  }

  \anchor{first antenna base end}{
    \pgf@process{\anchorA}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.2cm%
  }

  \anchor{first antenna}{
    %\csname pgf@anchor@mimoone@first antenna base start\endcsname
    \pgf@process{\anchorA}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.4cm%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    % \pgfpathrectanglecorners{\southwest}{\northeast}
    \pgfpathrectanglecorners
    { % First corner of the rectangle
      \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
    }
    { % Second corner of the rectangle
      \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    }

    %%%%%%% Draw the first antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorA}
    % The mimoshapesdrawantenna command only needs that the pgf@x and pgf@y
    % variables are correctly set. This is done by calling the anchor A
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of mimoone shape declaration xxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx mimotwo shape declaration xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{mimotwo}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimoone
  \inheritsavedanchors[from=mimoone]  
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define some savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we redefine the "anchorA", since it will be different from the
  % one we inherited from the mimoone shape.
  %
  % This anchor position will depend if the "left antennas" option was
  % passed or not.
  \savedanchor{\anchorA}{
    % -----> y position for the first antenna
    \pgf@y=.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.4\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }

  % Now we define a new anchorB for the second antenna.
  % This anchor position will depend if the "left antennas" option was
  % passed or not
  \savedanchor{\anchorB}{
    % -----> y position for the first antenna
    \pgf@y=-.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{-\pgfshapeminheight}
    \ifdim\pgf@y>.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.6\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimoone xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=mimoone]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Inherit normal anchors from mimoone xxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=mimoone]{center}
  \inheritanchor[from=mimoone]{north}
  \inheritanchor[from=mimoone]{east}
  \inheritanchor[from=mimoone]{south}
  \inheritanchor[from=mimoone]{west}
  \inheritanchor[from=mimoone]{north east}
  \inheritanchor[from=mimoone]{north west}
  \inheritanchor[from=mimoone]{south west}
  \inheritanchor[from=mimoone]{south east}
  \inheritanchor[from=mimoone]{text}
  \inheritanchor[from=mimoone]{A}
  \inheritanchor[from=mimoone]{first antenna base start}
  \inheritanchor[from=mimoone]{first antenna base end}
  \inheritanchor[from=mimoone]{first antenna}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{B}{
    \pgf@process{\anchorB}
  }

  \anchor{second antenna base start}{
    \pgf@process{\anchorB}
  }

  \anchor{second antenna base end}{
    \pgf@process{\anchorB}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.2cm%
  }

  \anchor{second antenna}{
    %\csname pgf@anchor@mimotwo@second antenna base start\endcsname
    \pgf@process{\anchorB}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.4cm%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    % \pgfpathrectanglecorners{\southwest}{\northeast}
    \pgfpathrectanglecorners
    { % First corner of the rectangle
      \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
    }
    { % Second corner of the rectangle
      \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    }

    %%%%%%% Draw the first antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorA}
    % The mimoshapesdrawantenna command only needs that the pgf@x and pgf@y
    % variables are correctly set. This is done by calling the anchor A
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    %%%%% Draw the second antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorB}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of mimotwo shape declaration xxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxx Mimo Shape with three antennas xxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{mimothree}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimotwo
  \inheritsavedanchors[from=mimotwo]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define some savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we redefine "anchorA" and "anchorB", since they will be different
  % from the one we inherited from the mimotwo shape.
  %
  % This anchor position will depend if the "left antennas" option was
  % passed or not.
  \savedanchor{\anchorA}{
    \pgf@y=.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.5\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }

  \savedanchor{\anchorC}{
    % y position for the first antenna
    \pgf@y=-.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{-\pgfshapeminheight}
    \ifdim\pgf@y>.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@y=0.9\pgf@y
    \advance\pgf@y by \antennayshift
    %
    % -----> x position
    \antennaStartXCoordinate
  }

  % B is in the middle of A and C
  \savedanchor{\anchorB}{
    % y position
    % First we get y position of anchor A
    \pgf@y=.5\ht\pgfnodeparttextbox
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@y<.5\pgf@ya
    \pgf@y=.5\pgf@ya
    \fi
    \pgf@ya=0.5\pgf@y
    % Then we get y position of anchor C
    \pgf@y=-.5\ht\pgfnodeparttextbox
    \setlength{\pgf@yc}{-\pgfshapeminheight}
    \ifdim\pgf@y>.5\pgf@yc
    \pgf@y=.5\pgf@yc
    \fi
    \pgf@yc=0.9\pgf@y
    % y position of anchor B is in the middle of anchor A and C
    \pgf@y=0.5\pgf@yc
    \advance\pgf@y by 0.5\pgf@ya
    %
    \advance\pgf@y by \antennayshift
    % 
    % x position
    \antennaStartXCoordinate
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimotwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=mimotwo]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from mimotwo xxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=mimotwo]{center}
  \inheritanchor[from=mimotwo]{north}
  \inheritanchor[from=mimotwo]{east}
  \inheritanchor[from=mimotwo]{south}
  \inheritanchor[from=mimotwo]{west}
  \inheritanchor[from=mimotwo]{north east}
  \inheritanchor[from=mimotwo]{north west}
  \inheritanchor[from=mimotwo]{south west}
  \inheritanchor[from=mimotwo]{south east}
  \inheritanchor[from=mimotwo]{text}
  \inheritanchor[from=mimotwo]{A}
  \inheritanchor[from=mimotwo]{B}
  \inheritanchor[from=mimotwo]{first antenna base start}
  \inheritanchor[from=mimotwo]{second antenna base start}
  \inheritanchor[from=mimotwo]{first antenna base end}
  \inheritanchor[from=mimotwo]{second antenna base end}
  \inheritanchor[from=mimotwo]{first antenna}
  \inheritanchor[from=mimotwo]{second antenna}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{C}{\anchorC}

  \anchor{third antenna base start}{
    \pgf@process{\anchorC}
  }
  \anchor{third antenna base end}{
    \pgf@process{\anchorC}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.2cm%
  }
  \anchor{third antenna}{
    %\csname pgf@anchor@mimothree@third antenna base start\endcsname
    \pgf@process{\anchorC}
    \advance\pgf@x by \antennaoffset%
    \advance\pgf@y by 0.4cm%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners
    { % First corner of the rectangle
      \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
    }
    { % Second corner of the rectangle
      \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    }

    %%%%%%% Draw the first antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorA}
    % The mimoshapesdrawantenna command only needs that the pgf@x and pgf@y
    % variables are correctly set. This is done by calling the anchor A
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    %%%%% Draw the second antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorB}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    %%%%% Draw the third %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorC}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  }
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of mimothree shape declaration xxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxx Mimo Shape with "many" antennas xxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{mimoind}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimothree
  \inheritsavedanchors[from=mimothree]

  % There is no need to define more savedanchors, since mimothree already
  % provide us with all we need.
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimotwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=mimothree]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from mimothree xxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=mimothree]{center}
  \inheritanchor[from=mimothree]{north}
  \inheritanchor[from=mimothree]{east}
  \inheritanchor[from=mimothree]{south}
  \inheritanchor[from=mimothree]{west}
  \inheritanchor[from=mimothree]{north east}
  \inheritanchor[from=mimothree]{north west}
  \inheritanchor[from=mimothree]{south west}
  \inheritanchor[from=mimothree]{south east}
  \inheritanchor[from=mimothree]{text}
  \inheritanchor[from=mimothree]{A}
  \inheritanchor[from=mimothree]{B}
  \inheritanchor[from=mimothree]{C}
  \inheritanchor[from=mimothree]{first antenna base start}
  \inheritanchor[from=mimothree]{second antenna base start}
  \inheritanchor[from=mimothree]{third antenna base start}
  \inheritanchor[from=mimothree]{first antenna base end}
  \inheritanchor[from=mimothree]{second antenna base end}
  \inheritanchor[from=mimothree]{third antenna base end}
  \inheritanchor[from=mimothree]{first antenna}
  \inheritanchor[from=mimothree]{second antenna}
  \inheritanchor[from=mimothree]{third antenna}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners
    { % First corner of the rectangle
      \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
    }
    { % Second corner of the rectangle
      \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    }

    %%%%%%% Draw the first antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Você pode usar \pgf@anchor@SHAPE_NAME@ANCHOR_NAME para mudar o \pgf@x
    % e o \pgf@y para as coordenadas de uma âncora. Só que se você resolver
    % mudar o nome do shape depois vai ter que mudar todas as linhas que
    % contem o SHAPE_NAME. Melhor usar o csname como na linha abaixo.
    \pgf@process{\anchorA}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    %%%%% Draw the second antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\csname pgf@anchor@\pgf@sm@shape@name @second antenna base end\endcsname
    \pgf@process{\anchorB}
    %\mimoshapesdrawantenna
    \drawellipses
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    %%%%% Draw the third antenna %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgf@process{\anchorC}
    \mimoshapesdrawantenna
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  }
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of mimoind shape declaration xxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxx Boxtwo Node xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{boxtwo}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimoone
  \inheritsavedanchors[from=mimoone]

  % There is no need to define more savedanchors, since mimoone already
  % provide us with all we need.
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimotwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=mimoone]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from mimoone xxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=mimotwo]{center}
  \inheritanchor[from=mimotwo]{north}
  \inheritanchor[from=mimotwo]{east}
  \inheritanchor[from=mimotwo]{south}
  \inheritanchor[from=mimotwo]{west}
  \inheritanchor[from=mimotwo]{north east}
  \inheritanchor[from=mimotwo]{north west}
  \inheritanchor[from=mimotwo]{south west}
  \inheritanchor[from=mimotwo]{south east}
  \inheritanchor[from=mimotwo]{text}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  % See section "Internals of How Point Commands Work" of the pgf manual to
  % understand pgf@process
  \anchor{A}{
    \pgf@process{\northeast}%
    \pgf@x=0pt
    \pgf@y=0.5\pgf@y%
  }

  \anchor{B}{
    \pgf@process{\northeast}%
    \pgf@x=0pt
    \pgf@y=-0.5\pgf@y%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    {
      \pgfpathrectanglecorners
      { % First corner of the rectangle
        \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
      }
      { % Second corner of the rectangle
        \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
      }
      \pgfusepath{stroke,fill}
    }
    
    % The two circles
    {
      \csname pgf@anchor@\pgf@sm@shape@name @A\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \csname pgf@anchor@\pgf@sm@shape@name @B\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/circle fill color}}
      \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/circle stroke color}}
      \pgfusepath{stroke,fill}
    }
  }
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx End of boxtwo shape declaration xxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx



%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxx Boxthree Node xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{boxthree}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % First we Inherit savedanchors (and savedmacro's) from mimoone
  \inheritsavedanchors[from=boxtwo]

  % There is no need to define more savedanchors, since mimoone already
  % provide us with all we need.
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from mimotwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=boxtwo]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from boxtwo xxxxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=boxtwo]{center}
  \inheritanchor[from=boxtwo]{north}
  \inheritanchor[from=boxtwo]{east}
  \inheritanchor[from=boxtwo]{south}
  \inheritanchor[from=boxtwo]{west}
  \inheritanchor[from=boxtwo]{north east}
  \inheritanchor[from=boxtwo]{north west}
  \inheritanchor[from=boxtwo]{south west}
  \inheritanchor[from=boxtwo]{south east}
  \inheritanchor[from=boxtwo]{text}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  % See section "Internals of How Point Commands Work" of the pgf manual to
  % understand pgf@process
  \anchor{A}{
    \northeast
    \pgf@x=0pt
    \pgf@y=0.6\pgf@y%
  }

  \anchor{B}{
    \pgf@x=0pt
    \pgf@y=0pt
  }

  \anchor{C}{
    \northeast
    \pgf@x=0pt
    \pgf@y=-0.6\pgf@y%
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Rectangle box
    {
      \pgfpathrectanglecorners
      { % First corner of the rectangle
        \pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}
      }
      { % Second corner of the rectangle
        \pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
      }
      \pgfusepath{stroke,fill}
    }
    
    % The three circles
    {
      \csname pgf@anchor@\pgf@sm@shape@name @A\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \csname pgf@anchor@\pgf@sm@shape@name @B\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \csname pgf@anchor@\pgf@sm@shape@name @C\endcsname
      \pgfcircle{\pgfpoint{\pgf@x}\pgf@y{}}{\pgfkeysvalueof{/pgf/circle radius}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/circle fill color}}
      \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/circle stroke color}}
      \pgfusepath{stroke,fill}
      }
  }
}

\makeatother


% The Comment below is only important for Emacs

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "testmimoshapes.tex"
%%% TeX-PDF-mode: t
%%% End: 
